Enhancing Video Summarization with Context Awareness

Video summarization is a crucial research area that aims to efficiently browse and retrieve relevant information from the vast amount of video content available today. With the exponential growth of multimedia data, the ability to extract meaningful representations from videos has become essential. Video summarization techniques automatically generate concise summaries by selecting keyframes, shots, or segments that capture the video's essence. This process improves the efficiency and accuracy of various applications, including video surveillance, education, entertainment, and social media. Despite the importance of video summarization, there is a lack of diverse and representative datasets, hindering comprehensive evaluation and benchmarking of algorithms. Existing evaluation metrics also fail to fully capture the complexities of video summarization, limiting accurate algorithm assessment and hindering the field's progress. To overcome data scarcity challenges and improve evaluation, we propose an unsupervised approach that leverages video data structure and information for generating informative summaries. By moving away from fixed annotations, our framework can produce representative summaries effectively. Moreover, we introduce an innovative evaluation pipeline tailored specifically for video summarization. Human participants are involved in the evaluation, comparing our generated summaries to ground truth summaries and assessing their informativeness. This human-centric approach provides valuable insights into the effectiveness of our proposed techniques. Experimental results demonstrate that our training-free framework outperforms existing unsupervised approaches and achieves competitive results compared to state-of-the-art supervised methods.

==> content/advisor-comment.tex <==
\chapter*{COMMENT OF THESIS'S ADVISOR}
\begin{tikzpicture}[remember picture, overlay]
  \draw[line width = 1pt] ($(current page.north west) + (1.2in,-1in)$) rectangle ($(current page.south east) + (-0.7in,1in)$);
\end{tikzpicture}
\multido{}{20}{\noindent\makebox[\linewidth]{\dotfill}\endgraf}

==> content/chap-background.tex <==
\chapter{Background}
\label{chapter:background}

\mycomment{chapter nay khong can thiet dau}

\begin{ChapAbstract}
    In this chapter, we provide a comprehensive overview of fundamental concepts in Machine Learning (\hyperref[section:back-machine]{Section \ref{section:back-machine}}) and Deep Learning (\hyperref[section:back-deep]{Section \ref{section:back-deep}}). Within each section, we introduce essential models that will be employed in the upcoming chapters. This foundational understanding is crucial for comprehending the subsequent chapters' content.  
\end{ChapAbstract}

\input{content/background/back-machine.tex}
\input{content/background/back-deep.tex}

==> content/experiment/exp-legacy.tex <==
\section{Evaluation methods}
\label{section:exp-evaluation}



\subsection{Quantitative evaluation}
\label{subsec:exp-evaluation-quantitative}
    Our quantitative evaluation compares the performance of the method that we proposed in \ref{section:method-model} with the baselines selected among previous works that were mentioned in \ref{chapter:related}. The datasets used for this comparison are already described in previous section \ref{section:exp-datasets}, hence this section is dedicated to the description of the evaluation metric and the baselines.

    

\subsection{Qualitative evaluation}
\label{subsec:exp-evaluation-qualitative}

    

==> content/reviewer-comment.tex <==
\chapter*{COMMENTS OF THESIS'S REVIEWER}
\begin{tikzpicture}[remember picture, overlay]
  \draw[line width = 1pt] ($(current page.north west) + (1.2in,-1in)$) rectangle ($(current page.south east) + (-0.7in,1in)$);
\end{tikzpicture}
\multido{}{20}{\noindent\makebox[\linewidth]{\dotfill}\endgraf}


==> content/syllabus.tex <==
\chapter{Project Proposal}
\begin{longtable}{|l|c|}
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Project title}: ENHANCING VIDEO SUMMARIZATION WITH CONTEXT AWARENESS
}\\
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Advisors}: Assoc. Prof. Trần Minh Triết (Faculty of Information Technology), Dr. Lê Trung Nghĩa (Faculty of Information Technology)} \\
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Duration}: January 1\textsuperscript{st}, 2023 to August 14\textsuperscript{th}, 2023}\\
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Students}: Huỳnh Lâm Hải Đăng (Student ID: 19125003) - Hồ Thị Ngọc Phượng (Student ID: 19125014)}\\
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Theme of Project}: theoretical research, proposed improvements.}\\
\hline
\multicolumn{2}{|m{\linewidth}|}{\textbf{Content}:\par
We aim to propose a novel approach for improving video summarization quality by integrating context awareness. We also aim to propose an evaluation metric that better suits the practical use of problem in real life.\par
The details include:
\begin{itemize}
  \item Literature Review and Proposal Writing \begin{itemize}
    \item Conduct a comprehensive literature review on video summarization, identifying the current state-of-the-art techniques and their limitations, as well as opportunities for improvement. 
    \item Analyze the importance of context in video summarization and compare existing methods and tools for context extraction in videos, in terms of performance and applicability for video summarization.
    \item Develop a research proposal, including research questions, hypothesis, and methodology, based on the findings from the literature review.
  \end{itemize}
\end{itemize}}\\
\hline

\multicolumn{2}{|m{\linewidth}|}{\begin{itemize}
  \item Dataset Collection \begin{itemize}
    \item Collect datasets suitable for training and testing.
    \item Analyze the current evaluation metrics for video summarization and identify their flaws.
    \item Define relevant performance metrics for evaluating the effectiveness of the context awareness in improving the quality of video summarization.
  \end{itemize}
  \item Model Development\begin{itemize}
    \item Develop baseline model for the sake of benchmarking.
    \item Develop different models to prove the proposed hypothesis.
    \item Train and optimize the model using the collected datasets.
  \end{itemize}
  \item Comparison with Existing Video Summarization Techniques\begin{itemize}
    \item Conduct experiments on proposed enhancements with a thoroughly designed ablation study.
    \item Analyze the strengths and weaknesses of the proposed approach.
    \item Conduct surveys based on the proposed evaluation metric.
  \end{itemize}
  \item Demo Application Development\begin{itemize}
    \item Develop a demo application that can demonstrate the functionality and usability of the proposed framework for video summarization.
  \end{itemize}
\end{itemize}}\\
\hline

\multicolumn{2}{|m{\linewidth}|}{\begin{itemize}
  \item Report Writing and Submission\begin{itemize}
    \item Write up the work, including an introduction, literature review, methodology, results, discussion, and conclusion.
  \end{itemize}
\end{itemize}}\\

\multicolumn{2}{|m{\linewidth}|}{
\textbf{Implementation plan}:
\begin{itemize}
  \item Literature Review and Proposal Writing: 01-01-2023 to 31-01-2023
  \item Dataset Collection: 01-02-2023 to 15-02-2023
  \item Saliency Detection Model Development: 16-02-2023 to 15-03-2023
  \item Video Summarization Model Development: 16-03-2023 to 15-04-2023
  \item Integration of Saliency Detection into Video Summarization: 16-04-2023 to 15-05-2023
  \item Comparison with Existing Video Summarization Techniques: 16-05-2023 to 31-05-2023
  \item Demo Application Development: 01-06-2023 to 30-06-2023
  \item Report Writing: 01-07-2023 to 31-07-2023
\end{itemize}}\\
\hline
\makecell{\\ \textbf{Advisors} \vspace*{2cm} \\ Assoc. Prof. Trần Minh Triết \vspace*{2cm} \\ Dr. Lê Trung Nghĩa} & \makecell{\textbf{HCMC, December 26\textsuperscript{th}, 2022}\\ \textbf{Authors} \vspace*{2cm} \\ Huỳnh Lâm Hải Đăng \vspace*{2cm} \\ Hồ Thị Ngọc Phượng}\\
\hline
\end{longtable}


==> eureka-pub.tex <==

A derivative paper of the research done in this work has been accepted to an international conference. The information about the accepted paper is detailed below:

\begin{itemize}
    \item \textbf{Paper}: H. Huynh-Lam, N. Ho-Thi, M. Tran, and T. Le, "Cluster-based Video Summarization with Temporal Context Awareness", in \ul{Pacific-Rim Symposium on Image and Video Technology (PSIVT)}, \textit{Accepted for Publication}, 2023.
\end{itemize}

